The sorting order on a Coxeter group

Let $(W,S)$ be an arbitrary Coxeter system. For each word $\omega$ in the generators we define a partial order--called the {\sf $\omega$-sorting order}--on the set of group elements $W_\omega\subseteq W$ that occur as subwords of $\omega$. We show that the $\omega$-sorting order is a supersolvable join-distributive lattice and that it is strictly between the weak and Bruhat orders on the group. Moreover, the $\omega$-sorting order is a "maximal lattice" in the sense that the addition of any collection of Bruhat covers results in a nonlattice. Along the way we define a class of structures called {\sf supersolvable antimatroids} and we show that these are equivalent to the class of supersolvable join-distributive lattices.

==> default <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 2169 6964 8086 7129
4 0 0 55 -1 0 10 0.0000 2 165 2190 5100 7084 $\\text{$\\omega_2$-sorting order}$\001
4 0 0 54 -1 0 10 0.0000 2 165 2190 3470 7084 $\\text{$\\omega_1$-sorting order}$\001
4 0 0 53 -1 0 10 0.0000 2 150 1350 6736 7084 $\\text{strong order}$\001
4 0 0 52 -1 0 10 0.0000 2 150 1260 2169 7084 $\\text{weak order}$\001
-6
6 3525 4125 4575 6975
6 3675 4800 4050 6225
4 0 0 51 -1 0 8 0.0000 2 105 360 3675 5550 $1200$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 3675 4950 $1210$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 3675 6150 $1000$\001
-6
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 4050 4350 36 36 4050 4350 4086 4350
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3600 4950 36 36 3600 4950 3636 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 4500 4950 36 36 4500 4950 4536 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 4500 5550 36 36 4500 5550 4536 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3600 5550 36 36 3600 5550 3636 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3600 6150 36 36 3600 6150 3636 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 4050 6750 36 36 4050 6750 4086 6750
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 4500 6150 36 36 4500 6150 4536 6150
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4050 6750 3600 6150
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4050 6750 4500 6150
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4500 6150 4500 5550
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4500 5550 4500 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 3600 6150 3600 5550
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 3600 5550 3600 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 3600 4950 4050 4350
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4050 4350 4500 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4500 6150 3600 5550
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 4500 5550 3600 4950
4 0 0 51 -1 0 8 0.0000 2 105 360 4125 6225 $0200$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 4125 5625 $0210$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 4125 5025 $0212$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 3900 6900 $0000$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 3900 4275 $1212$\001
-6
6 6525 4275 7575 6825
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 7500 4950 36 36 7500 4950 7536 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 7050 4350 36 36 7050 4350 7086 4350
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6600 4950 36 36 6600 4950 6636 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6600 5550 36 36 6600 5550 6636 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6600 6150 36 36 6600 6150 6636 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 7500 6150 36 36 7500 6150 7536 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 7500 5550 36 36 7500 5550 7536 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 7050 6750 36 36 7050 6750 7086 6750
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7050 6750 6600 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7050 6750 7500 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 6600 6150 6600 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 6600 5550 6600 4950
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 6600 4950 7050 4350
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7050 4350 7500 4950
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7500 4950 7500 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7500 5550 7500 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7500 6150 6600 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 6600 5550 7500 4950
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 6600 4950 7500 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 7500 5550 6600 6150
-6
6 5175 4875 5550 6300
4 0 0 51 -1 0 8 0.0000 2 105 360 5175 5625 $1200$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 5175 5025 $1210$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 5175 6225 $1000$\001
-6
6 5625 4800 6000 6225
4 0 0 51 -1 0 8 0.0000 2 105 360 5625 6150 $0200$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 5625 5550 $0210$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 5625 4950 $0212$\001
-6
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 2550 4350 36 36 2550 4350 2586 4350
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 2100 4950 36 36 2100 4950 2136 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3000 4950 36 36 3000 4950 3036 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 2100 5550 36 36 2100 5550 2136 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3000 5550 36 36 3000 5550 3036 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 3000 6150 36 36 3000 6150 3036 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 2100 6150 36 36 2100 6150 2136 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 2550 6750 36 36 2550 6750 2586 6750
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 5550 4350 36 36 5550 4350 5586 4350
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 5100 4950 36 36 5100 4950 5136 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6000 4950 36 36 6000 4950 6036 4950
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6000 5550 36 36 6000 5550 6036 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 5100 5550 36 36 5100 5550 5136 5550
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 5100 6150 36 36 5100 6150 5136 6150
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 5550 6750 36 36 5550 6750 5586 6750
1 3 0 1 0 7 49 -1 20 0.000 1 0.0000 6000 6150 36 36 6000 6150 6036 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2550 6750 2100 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2550 6750 3000 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 3000 6150 3000 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 3000 5550 3000 4950
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2100 6150 2100 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2100 5550 2100 4950
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2100 4950 2550 4350
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 2550 4350 3000 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5550 6750 6000 6150
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 6000 6150 6000 5550
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 6000 5550 6000 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5100 6150 5100 5550
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5100 5550 5100 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5100 4950 5550 4350
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5550 4350 6000 4950
2 1 0 2 0 7 51 -1 -1 0.000 1 1 -1 0 0 2
	 5562 6750 5112 6150
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 5100 6150 6000 5550
2 1 0 2 0 7 51 -1 20 0.000 1 1 -1 0 0 2
	 5100 5550 6000 4950
4 0 0 51 -1 0 8 0.0000 2 105 360 5400 6900 $0000$\001
4 0 0 51 -1 0 8 0.0000 2 105 360 5400 4275 $1212$\001

